The Saga of M81: Global View of a Massive Stellar Halo in Formation

Recent work has shown that Milky Way-mass galaxies display an incredible range of stellar halo properties, yet the origin of this diversity is unclear. The nearby galaxy M81 $-$ currently interacting with M82 and NGC 3077 $-$ sheds unique light on this problem. We present a Subaru Hyper Suprime-Cam survey of the resolved stellar populations around M81, revealing M81's stellar halo in never-before-seen detail. We resolve the halo to unprecedented $V$-band equivalent surface brightnesses of 33 mag arcsec$^{-2}$, and produce the first-ever global stellar mass density map for a Milky Way-mass stellar halo outside of the Local Group. Using the minor axis, we confirm M81's halo as one of the lowest mass and metal-poorest known ($M_{\star} \simeq 1.16{\times}10^9 M_{\odot}$, [Fe/H] $\simeq {-}1.2$) $-$ indicating a relatively quiet prior accretion history. Yet, our global halo census finds that tidally unbound material from M82 and NGC 3077 provides a substantial infusion of metal-rich material ($M_{\star} \simeq 5.4{\times}10^8$ $M_{\odot}$, [Fe/H] $\simeq {-}$0.9). We further show that, following the accretion of its massive satellite M82 (and the LMC-like NGC 3077), M81 will host one of the most massive and metal-rich stellar halos in the nearby universe. Thus, the saga of M81: following a passive history, M81's merger with M82 will completely transform its halo from a low-mass, anemic halo rivaling the MW, to a metal-rich behemoth rivaled only by systems such as M31. This dramatic transformation indicates that the observed diversity in stellar halo properties is primarily driven by diversity in the largest mergers these galaxies have experienced.

==> minax_profiles.tex <==
\newcolumntype{p}{!{\extracolsep{50pt}}c!{\extracolsep{0pt}}}

\begin{deluxetable}{ppp}
\tablewidth{0.48\linewidth}
\tablecaption{Minor Axis SB \& Color Profiles\label{tab:minax}}
\tablecolumns{3}
\tabletypesize{\small}
\tablehead{% 
\vspace{-5pt}
\colhead{$R$} & 
\colhead{$\mu_{V}$} & 
\colhead{$g{-}i$} \\ \vspace{-15pt}
%%%
\colhead{(kpc)} & 
\colhead{(\magsqarc)} & 
\colhead{(mag)} \\
}
%
\startdata
10 & 28.02\,$\pm$\,1.46 & 1.99$^{{-}0.13}_{{+}0.02}$ \\ 
12 & 28.23\,$\pm$\,1.02 & 1.94$^{{-}0.09}_{{+}0.02}$ \\ 
14 & 28.71\,$\pm$\,0.66 & 1.89$^{{-}0.09}_{{+}0.02}$ \\ 
16 & 29.26\,$\pm$\,0.45 & 1.90$^{{-}0.09}_{{+}0.02}$ \\ 
18 & 29.52\,$\pm$\,0.44 & 1.78$^{{-}0.04}_{{+}0.02}$ \\ 
20 & 30.27\,$\pm$\,0.34 & 1.79$^{{-}0.05}_{{+}0.02}$ \\ 
22 & 30.75\,$\pm$\,0.29 & 1.79$^{{-}0.02}_{{+}0.02}$ \\ 
24 & 31.13\,$\pm$\,0.31 & 1.75$^{{-}0.02}_{{+}0.02}$ \\ 
26 & 31.75\,$\pm$\,0.31 & 1.76$^{{-}0.02}_{{+}0.02}$ \\ 
28 & 31.93\,$\pm$\,0.32 & 1.72$^{{-}0.02}_{{+}0.02}$ \\ 
30 & 32.13\,$\pm$\,0.33 & 1.71$^{{-}0.02}_{{+}0.02}$ \\ 
32 & 32.54\,$\pm$\,0.35 & 1.70$^{{-}0.02}_{{+}0.02}$ \\ 
34 & 32.51\,$\pm$\,0.34 & 1.67$^{{-}0.02}_{{+}0.02}$ \\ 
36 & 32.32\,$\pm$\,0.34 & 1.70$^{{-}0.02}_{{+}0.02}$ \\ 
38 & 32.69\,$\pm$\,0.36 & 1.71$^{{-}0.02}_{{+}0.02}$ \\ 
40 & 32.64\,$\pm$\,0.35 & 1.69$^{{-}0.02}_{{+}0.02}$ \\ 
45 & 33.18\,$\pm$\,0.39 & 1.71$^{{-}0.02}_{{+}0.02}$ \\ 
50 & 33.60\,$\pm$\,0.42 & 1.72$^{{-}0.02}_{{+}0.02}$ \\ 
55 & 34.10\,$\pm$\,0.45 & 1.67$^{{-}0.03}_{{+}0.03}$ \\ 
60 & 34.46\,$\pm$\,0.48 & 1.68$^{{-}0.02}_{{+}0.02}$ \\ 
\vspace{-8pt}
\enddata
\tablecomments{The radial minor axis average surface brightness and average $g{-}i$\ color profiles as shown in Figure \ref{fig:minax-sb} \& \ref{fig:minax-color}. See \S\,\ref{sec:sb-prof} and \S\,\ref{sec:color-prof} for discussion of how the measurements and uncertainties are computed.}
\end{deluxetable}
